Structured Pruning of Neural Networks for Constraints Learning

In recent years, the integration of Machine Learning (ML) models with Operation Research (OR) tools has gained popularity across diverse applications, including cancer treatment, algorithmic configuration, and chemical process optimization. In this domain, the combination of ML and OR often relies on representing the ML model output using Mixed Integer Programming (MIP) formulations. Numerous studies in the literature have developed such formulations for many ML predictors, with a particular emphasis on Artificial Neural Networks (ANNs) due to their significant interest in many applications. However, ANNs frequently contain a large number of parameters, resulting in MIP formulations that are impractical to solve, thereby impeding scalability. In fact, the ML community has already introduced several techniques to reduce the parameter count of ANNs without compromising their performance, since the substantial size of modern ANNs presents challenges for ML applications as it significantly impacts computational efforts during training and necessitates significant memory resources for storage. In this paper, we showcase the effectiveness of pruning, one of these techniques, when applied to ANNs prior to their integration into MIPs. By pruning the ANN, we achieve significant improvements in the speed of the solution process. We discuss why pruning is more suitable in this context compared to other ML compression techniques, and we identify the most appropriate pruning strategies. To highlight the potential of this approach, we conduct experiments using feed-forward neural networks with multiple layers to construct adversarial examples. Our results demonstrate that pruning offers remarkable reductions in solution times without hindering the quality of the final decision, enabling the resolution of previously unsolvable instances.

==> tikz_nn.tex <==
\begin{figure}
    \centering

\scalebox{0.6}{
\begin{tikzpicture}[x=2.7cm,y=1.6cm]
  \message{^^JNeural network activation}
  \def\NI{3} % number of nodes in input layers
  \def\NH{4} % number of nodes in hidden layers
  \def\NN{4} % number of nodes in hidden layers
  \def\NO{2} % number of nodes in output layers
  \def\yshift{0.0} % shift last node for dots
  
  % INPUT LAYER
  \foreach \i [evaluate={\c=int(\i==\NI); \y=\NI/2-\i-\c*\yshift; \index=(\i<\NI?int(\i):"n");}]
              in {1,...,\NI}{ % loop over nodes
    \node[node black,outer sep=0.6] (NI-\i) at (0,\y) {};
  }

    % Hidden LAYER 1
  \foreach \i [evaluate={\c=int(\i==\NH); \y=\NH/2-\i-\c*\yshift; \index=(\i<\NH?int(\i):"m");}]
    in {\NH,...,1}{ % loop over nodes
      \node[node green]
        (NH-\i) at (1,\y) {};
      \foreach \j in {1,...,\NI}{ % loop over nodes in previous layer
        %\draw[connect,white,line width=1.2] (NI-\j) -- (NO-\i);
        \draw[connect,myblue!20] (NI-\j) -- (NH-\i);
      }
  }
  

      % Hidden LAYER 2
  \foreach \i [evaluate={\c=int(\i==\NN); \y=\NN/2-\i-\c*\yshift; \index=(\i<\NN?int(\i):"m");}]
    in {\NN,...,1}{ % loop over nodes
    \ifnum\i=1 % high-lighted node
      \node[node yellow]
        (NN-\i) at (2,\y) {};
      \foreach \j [evaluate={\index=(\j<\NH?int(\j):"n");}] in {1,...,\NH}{ % loop over nodes in previous layer
        \draw[connect,white,line width=1.2] (NH-\j) -- (NN-\i);
        \draw[connect] (NH-\j) -- (NN-\i)
          node[pos=0.50] {\contour{white}{}};
      }
    \else % other light-colored nodes
      \node[node yellow]
        (NN-\i) at (2,\y) {};
      \foreach \j in {1,...,\NH}{ % loop over nodes in previous layer
        %\draw[connect,white,line width=1.2] (NI-\j) -- (NO-\i);
        \draw[connect,myblue!20] (NH-\j) -- (NN-\i);
      }
    \fi
  }

    % OUTPUT LAYER
  \foreach \i [evaluate={\c=int(\i==\NO); \y=\NO/2-\i-\c*\yshift; \index=(\i<\NO?int(\i):"m");}]
    in {\NO,...,1}{ % loop over nodes
   
      \node[node blue]
        (NO-\i) at (3,\y) {};
      \foreach \j [evaluate={\index=(\j<\NN?int(\j):"n");}] in {1,...,\NN}{ % loop over nodes in previous layer
      \ifnum\j=1 % high-lighted node
        \draw[connect,white,line width=1.2] (NN-\j) -- (NO-\i);
        \draw[connect] (NN-\j) -- (NO-\i)
          node[pos=0.50] {\contour{white}{}};

    \else % other light-colored nodes
        \draw[connect,myblue!20] (NN-\j) -- (NO-\i);
    \fi
    }
  }
% \node[red] at (NN-1) {Q};
\end{tikzpicture}
}

    \caption{Corresponding network, the highlighted part is the pruned one.}
    \label{fig:net_pruned}
\end{figure}
